Lookback Lens: Detecting and Mitigating Contextual Hallucinations in Large Language Models Using Only Attention Maps

When asked to summarize articles or answer questions given a passage, large language models (LLMs) can hallucinate details and respond with unsubstantiated answers that are inaccurate with respect to the input context. This paper describes a simple approach for detecting such contextual hallucinations. We hypothesize that contextual hallucinations are related to the extent to which an LLM attends to information in the provided context versus its own generations. Based on this intuition, we propose a simple hallucination detection model whose input features are given by the ratio of attention weights on the context versus newly generated tokens (for each attention head). We find that a linear classifier based on these lookback ratio features is as effective as a richer detector that utilizes the entire hidden states of an LLM or a text-based entailment model. The lookback ratio-based detector -- Lookback Lens -- is found to transfer across tasks and even models, allowing a detector that is trained on a 7B model to be applied (without retraining) to a larger 13B model. We further apply this detector to mitigate contextual hallucinations, and find that a simple classifier-guided decoding approach is able to reduce the amount of hallucination, for example by 9.6% in the XSum summarization task.

==> tables/mt-bench.tex <==
\begin{table}[h!]
\centering
\small
\begin{tabular}{lcc}
\toprule
\multirow{2}{*}{\bf Method} & \multicolumn{2}{c}{\bf MT Bench} \\
\cmidrule(lr){2-3}
\multirow{2}{*}{} & \bf Hallu. & \bf Original \\
\midrule
\bf Greedy Decoding & 5.66 & 5.10 \\
\midrule
\multicolumn{3}{c}{\it Classifier Guided Sampling (8 candidates)} \\
\midrule
\bf Ours LR Clf. & \bf 6.12 & 5.10 \\
\bf Hiddens Clf. & 5.04 & 5.06 \\
\bf SoTA NLI Clf. & 5.98 & 5.03 \\
\bottomrule
\end{tabular}
\caption{Performance Comparison on MT Bench Dataset using Different Methods and Chunk Sizes}
\label{tab:mtbench}
\end{table}

==> tables/qualitative-example.tex <==
\begin{table*}[h]
\small
\centering
\caption{Qualitative example on XSum using 7B model.}
\label{tab:qualitative_example}
\begin{tabular}{p{0.08\linewidth}p{0.35\linewidth}p{0.4\linewidth}}
\toprule
Document & \multicolumn{2}{l}{
\begin{minipage}{0.8\linewidth}
She had the "biggest year of her career", playing 95 shows, bringing in an average \$2.4m (£1.5m) per city, according to Forbes. \\
Endorsement deals with companies like Pepsi and H\&M, along with the surprise album she released in December 2013, helped her to the top spot.\\
The self-titled album was released on iTunes with no prior promotion.\\
Beyonce has just announced she'll be releasing a platinum version of that album later this month, which will include new songs and a concert video.\\
Source: Forbes\\
Taylor Swift came in second on the Forbes list, taking home an estimated \$64m (£40m).\\
Completing the top three is Pink, who played 85 dates during the time period Forbes used to make its estimates.\\
Her earnings were valued at \$52m (£32.5m).\\
Other artists on the list include Rihanna in fourth with \$48m (£30m) and Katy Perry, who took home \$40m (£25m), in fifth.\\
Forbes calculated earnings by looking at income from "touring, record sales, publishing, merchandise sales, endorsements and other ventures" between June 2013 and June 2014.\\
They also interviewed managers, lawyers and executives and looked at data from organisations such as Nielsen SoundScan.\\
Some of the high-profile artists who missed out on a spot in the top 10 included Madonna, Nicki Minaj and Alicia Keys.\\
Follow @BBCNewsbeat on Twitter and Radio1Newsbeat on YouTube
\end{minipage}}\\
\midrule
Greedy Decoding & \multicolumn{2}{p{0.8\linewidth}}{Beyonce topped the Forbes list of highest-paid female musicians, earning an estimated \$100m (£64m) in the past year.} \\
\midrule
\multirow[m]{5}{0.08\linewidth}{Ours Step1} & \multicolumn{2}{p{0.8\linewidth}}{1. According to Forbes, Beyonce had the biggest year of her career in terms (0.99)} \\
& \multicolumn{2}{p{0.8\linewidth}}{2. According to Forbes, Beyonce came in first place on their list of highest (0.97)} \\
 & \multicolumn{2}{p{0.8\linewidth}}{\dots} \\
 &  \multicolumn{2}{p{0.8\linewidth}}{7. According to Forbes, Beyonce earned an estimated \$30m (£ (0.65)} \\
 & \multicolumn{2}{p{0.8\linewidth}}{8. Beyonce became the highest-paid female musician in the world in the (0.42)} \\
\midrule
\multicolumn{3}{p{\linewidth}}{\dots} \\
\midrule
\multirow[m]{5}{0.08\linewidth}{Ours Step3} & \multirow[m]{5}{0.6\linewidth}{According to Forbes, Beyonce had the biggest year of her career in terms of earnings, bringing in an average of \$2.4m per city} & 1. , thanks to endorsement deals and her surprise album. Taylor Swift came (0.94) \\
& & 2. through 95 shows, with endorsement deals and a surprise album (0.87) \\
 & & \dots \\
 & &  3. and earning an estimated \$80m overall. Endorsement deals (0.12) \\
 & &  4. and earning an estimated \$100m overall. (0.05) \\
\midrule
\end{tabular}
\end{table*}
